Conservation laws for Electron Vortices in Strong-Field Ionisation

We investigate twisted electrons with a well defined orbital angular momentum, which have been ionised via a strong laser field. By formulating a new variant of the well-known strong field approximation, we are able to derive conservation laws for the angular momenta of twisted electrons in the cases of linear and circularly polarised fields. In the case of linear fields, we demonstrate that the orbital angular momentum of the twisted electron is determined by the magnetic quantum number of the initial bound state. The condition for the circular field can be related to the famous ATI peaks, and provides a new interpretation for this fundamental feature of photoelectron spectra. We find the length of the circular pulse to be a vital factor in this selection rule and, employing an effective frequency, we show that the photoelectron OAM emission spectra is sensitive to the parity of the number of laser cycles. This work provides the basic theoretical framework with which to understand the OAM of a photoelectron undergoing strong field ionisation.

==> 2021_07_70_The Paper Draft for OAM/Authors.tex <==
\author{Yuxin Kang\inst{1} \and 
	Emilio Pisanty\orcid{0000-0003-0598-8524}\inst{2,3} \and
	Marcelo Ciappina\orcid{0000-0002-1123-6460}\inst{3,4,5} \and
	Maciej Lewenstein\orcid{0000-0002-0210-7800}\inst{3,6} \and
	Carla Figueira de Morisson Faria\orcid{0000-0001-8397-4529}\inst{1} \and
	Andrew S Maxwell\orcid{0000-0002-6503-4661}\inst{1,3}
}
	
% \thanks is optional - remove next line if not needed
%\thanks{\emph{Present address:} Insert the address here if needed}%
%}                     % Do not remove
%
%\offprints{}          % Insert a name or remove this line
%
\institute{Department of Physics \& Astronomy, University College London, Gower Street, London WC1E 6BT, United Kingdom
	\and
%
Max Born Institute for Nonlinear Optics and Short Pulse Spectroscopy, Max-Born-Stra{\ss}e 2A, Berlin 12489, Germany
\and
%
ICFO - Institut de Ciencies Fotoniques, The Barcelona Institute of Science and Technology, Av. Carl Friedrich Gauss 3, 08860 Castelldefels (Barcelona), Spain
\and
%
Physics Program, Guangdong Technion -- Israel Institute of Technology, Shantou, Guangdong 515063, China
\and
%
Technion -- Israel Institute of Technology, Haifa, 32000, Israel
\and
%
ICREA, Pg. Lluís Companys 23, 08010 Barcelona, Spain
}
%

==> 2021_07_70_The Paper Draft for OAM/SF_Def.tex <==
\newcommand{\figref}[1]{\figurename~\ref{#1}}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
\newcommand{\Schr}{Schr\"odinger }
\newcommand{\ip}{\mathrm{I}_\mathrm{p}}
\newcommand{\up}{\mathrm{U}_\mathrm{p}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\rbh}{\hat{\mathbf{r}}}
\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\grad}{\mathbf{\nabla}}
\renewcommand\Re{\mathrm{Re}}
\renewcommand\Im{\mathrm{Im}}
\newcommand{\erf}{\;\mathrm{erf}}
\newcommand{\mel}[3]{\braket{#1|#2|#3}}
\newcommand{\sgn}{\mathrm{sgn}}

\newcommand*\conj[1]{\overline{#1}}

==> 2021_07_70_The Paper Draft for OAM/orcidicon.tex <==


\newcommand{\orcid}[1]{%
  ~\href{https://orcid.org/#1}{\includegraphics[width=8pt]{Figures/ORCID-icon.png}}%
  }

\newcommand{\linkedorcid}[1]{\href{https://orcid.org/#1}{#1}}
% \newcommand{\orcid}[1]{}
